Revisiting Structured Dropout

Large neural networks are often overparameterised and prone to overfitting, Dropout is a widely used regularization technique to combat overfitting and improve model generalization. However, unstructured Dropout is not always effective for specific network architectures and this has led to the formation of multiple structured Dropout approaches to improve model performance and, sometimes, reduce the computational resources required for inference. In this work, we revisit structured Dropout comparing different Dropout approaches to natural language processing and computer vision tasks for multiple state-of-the-art networks. Additionally, we devise an approach to structured Dropout we call \textbf{\emph{ProbDropBlock}} which drops contiguous blocks from feature maps with a probability given by the normalized feature salience values. We find that with a simple scheduling strategy the proposed approach to structured Dropout consistently improved model performance compared to baselines and other Dropout approaches on a diverse range of tasks and models. In particular, we show \textbf{\emph{ProbDropBlock}} improves RoBERTa finetuning on MNLI by $0.22\%$, and training of ResNet50 on ImageNet by $0.28\%$.

==> sections/setup.tex <==
\section{Experiments}
In the following section, we lay out the experimental setup for this paper and briefly discuss the datasets and models considered. To properly assess our approach to structured Dropout we test both vision and language tasks for state-of-the-art models. 

We compare the performance of models trained with the proposed ProbDropBlock approach to those trained with other forms of Dropout and baseline models trained without any form of Dropout.

\subsection{Setup}
In this work, we considered six datasets, 3 NL (natural language) datasets and 3 CV (computer vision) datasets. The NL datasets considered are all part of \textbf{GLUE} - the multitask benchmark and analysis platform for natural language understanding \cite{GLUE} and the CV datasets are widely accepted and used within the CV community.
